m&m's: A Benchmark to Evaluate Tool-Use for multi-step multi-modal Tasks

Real-world multi-modal problems are rarely solved by a single machine learning model, and often require multi-step computational plans that involve stitching several models. Tool-augmented LLMs hold tremendous promise for automating the generation of such computational plans. However, the lack of standardized benchmarks for evaluating LLMs as planners for multi-step multi-modal tasks has prevented a systematic study of planner design decisions. Should LLMs generate a full plan in a single shot or step-by-step? Should they invoke tools directly with Python code or through structured data formats like JSON? Does feedback improve planning? To answer these questions and more, we introduce m&m's: a benchmark containing 4K+ multi-step multi-modal tasks involving 33 tools that include multi-modal models, (free) public APIs, and image processing modules. For each of these task queries, we provide automatically generated plans using this realistic toolset. We further provide a high-quality subset of 1,565 task plans that are human-verified and correctly executable. With m&m's, we evaluate 10 popular LLMs with 2 planning strategies (multi-step vs. step-by-step planning), 2 plan formats (JSON vs. code), and 3 types of feedback (parsing/verification/execution). Finally, we summarize takeaways from our extensive experiments. Our dataset and code are available on HuggingFace (https://huggingface.co/datasets/zixianma/mnms) and Github (https://github.com/RAIVNLab/mnms).

==> figures/exec_acc_vs_others.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/exec_acc_vs_others.pdf}
    \caption{\textbf{Execution results accuracy vs. other metrics.} We find a strong positive correlation between the execution results accuracy and our main metrics, including tool-F1, argname-F1, and pass rate, with Pearson correlation coefficients $r=0.77, 0.73, 0.95$ respectively.}
    \label{fig:exec_acc_vs_others}
\end{figure}

==> figures/plan_system.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/plan_system.pdf}
    \caption{We implemented a planning system with four modules.}
    \label{fig:plan-system}
\end{figure}

==> figures/tool_frequency_before.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{images/tool_frequency_before.pdf}
    \caption{\textbf{Tool frequency before balancing.} }
    \label{fig:tool-freq-before}
\end{figure}

==> old_sections/01_introduction_v1.tex <==
\section{Introduction}
Humans are excellent at problem-solving and capable of completing a wide range of tasks, ranging from everyday tasks such as navigation, and cleaning to much more complex ones such as data analysis and travel planning.  By contrast, most state-of-the-art machine learning models have focused on simpler tasks but struggle to solve complex ecologically valid human tasks. Psychology literature reveals that the key to human problem-solving lies in decomposition: People rarely complete tasks in their entirety. Instead, they decompose complex tasks into subtasks that are easier to tackle ~\cite{correa2023humans,allen2020rapid}. In addition, tool use...
% Inspired by this insight, machine learning researchers have recently proposed to automate diverse tasks by using large language models to decompose complex tasks into simpler subtasks and solve each of the subtasks using appropriate tools. 
% While these works all involve tool use and are related to each other, they focus on different aspects of language models' tool use capabilities. For example, some focus on LLMs' abilities to use tools to solve visual-linguistic tasks such as VQA, while others only evaluate LLMs' abilities to use public APIs or HuggingFace models. They also formulate the problems differently, some as natural language or pseudo-code generation while others as code generation. No work has systematically studied or compared LLMs' tool use abilities using the same framework. Therefore, we are curious: what are the best practices for using LLMs to plan over complex tasks and solve them with tools (if any)? 

(Task decomposition) and tool use are key to human problem-solving, and researchers have shown that tool-augmented LLMs have the potential to solve a wide range of tasks. 

% Toolformer was one of the first few works that proposed to augment large language models with tools and showed that language models can be finetuned to learn when and how to call external tools such as a calculator or a search engine. Similarly, ToolLlama finetuned the open-source large language model Llama on an instruction-tuning dataset for tool use. Apart from finetuning, several other works have also demonstrated that large language models' in-context learning ability can be leveraged for tool use.  For example, Visprog proposes to solve complex and compositional visual tasks by few-shot prompting large language models to generate python-like modular programs. Similarly, ViperGPT leverages code-generation models to compose vision-and-language models into subroutines to solve complex visual tasks. More recently, HuggingGPT has demonstrated that large language models can act as central planners and answer complex user queries by calling multimodal models in HuggingFace. \\

In addition, feedback is important to human problem solving too, and has been shown to help LLMs with reasoning tasks. For example, ...

Despite the benefits of feedback, few works have studied LLMs' task decomposition and tool use abilities with feedback. ReACT is one of the first works that incorporates execution feedback as input to language models. Building upon ReACT, ToolLlama proposes a better prompting strategy DFSDT for tool use that also involves external feedback. However, these works are limited in two major ways. First, they formulate task planning as a step-by-step action/tool prediction problem, which can be time and cost-inefficient and even impractical when only models with short context length are accessible. Second, they only consider external feedback from an execution module, which could be time-consuming and even dangerous to run in safety-critical applications. 

Thus, we wonder: can feedback improve large language models' tool use performance in other settings beyond single-step prediction such as multi-step prediction (as proposed in HuggingGPT)? And are there other types of feedback, such as verification feedback, helpful for language models' to plan over complex tasks and use tools to solve them?

To answer these questions, we propose a unified framework along with a new benchmark \name for studying LLMs' abilities to decompose multi-modal tasks and use multi-domain tools to solve them. Concretely, we make the following three contributions:
\begin{enumerate}
    \item We contribute a novel benchmark with realistic user requests that require tools across three domains -- multimodal ML models, public APIs, and data processing modules -- to solve as well as human-verified solutions to these requests; 
    % 2) it supports evaluation of planners on ambiguous requests by adding alternative plans to the label set;
    \item We establish a framework to systematically study LLM's few-shot tool use abilities in two different settings (multi-step vs. single-step prediction) with two action formulations (natural language vs. code) as well as different types of feedback (verification, execution, or both).
    \item With this novel dataset and comprehensive framework, we benchmark the abilities of 10+ state-of-the-art chat-LLMs with varying sizes to plan over complex multi-modal tasks and solve them with diverse tools across multiple domains.
\end{enumerate}
Through extensive experiments, we learned the following X takeaways: first, ReACT-style single-step prediction can lead to better tool use performance than multi-step prediction at the cost of token efficiency; second, both verification and execution feedback can improve chat-LLMs' tool use performance by up to X \%; third, something about code vs. json-format natural language generation.  





==> old_sections/01_introduction_v2.tex <==
\section{Introduction}
\input{figures/dataset_examples}
Humans are excellent at problem-solving and capable of completing a wide range of tasks, ranging from everyday tasks such as navigation, and cleaning to much more complex ones such as data analysis and travel planning.  By contrast, most state-of-the-art machine learning models have focused on simpler tasks but struggle to solve complex ecologically valid human tasks. Psychology literature reveals that the key to human problem-solving lies in decomposition: People rarely complete tasks in their entirety. Instead, they decompose complex tasks into subtasks that are easier to tackle ~\cite{correa2023humans,allen2020rapid}. 

Inspired by this insight, machine learning researchers have recently proposed to automate diverse tasks by using large language models to decompose complex tasks into simpler subtasks and solve each of the subtasks using appropriate tools \cite{schick2024toolformer, yao2023react, qin2023toolllm, gupta2022visual, suris2023vipergpt, shen2023hugginggpt}. Several works demonstrate that we can leverage large language models' in-context learning ability for task decomposition and planning.  For example, ReACT proposes a prompting method to help language models reason about and generate step-by-step action plans for challenging linguistic and decision-making tasks\cite{yao2023react}. Visprog proposes to solve compositional visual tasks by prompting large language models to generate python-like modular programs\cite{gupta2022visual}. Similarly, ViperGPT leverages code-generation models to compose vision-and-language models into subroutines to solve complex visual tasks \cite{suris2023vipergpt}. More recently, HuggingGPT demonstrates that large language models can act as central planners and answer complex user queries by calling multimodal models in HuggingFace\cite{shen2023hugginggpt}. Apart from in-context learning, a few works have also finetuned language models to be better at task planning and tool use. Toolformer proposes to augment large language models with tools and show that language models can be finetuned to learn when and how to call external tools such as a calculator or a search engine \cite{schick2024toolformer}. Similarly, ToolLlama instruction-tunes Llama for tool use and demonstrates better performance than Llama \cite{qin2023toolllm}. 

While all these works involve task planning and tool use, they focus on different task and tool space and evaluate large language models on different benchmarks. For example, ReACT evaluates large language models' abilities to perform linguistic and decision-making tasks using existing benchmarks such as HotpotQA and WebShop. 
Visprog and ViperGPT test large language models' abilities to solve visual-linguistic tasks \cite{gupta2022visual, suris2023vipergpt} with vision-language models and image processing modules on various benchmarks, including GQA, RefCOCO, and NLVR etc. (cite). On the other hand, ToolLlama proposes a new benchmark called ToolBench for evaluating language models' abilities to call public APIs for daily life queries \cite{qin2023toolllm, yao2023react}. More recently, a few works such as ToolEmu, TaskBench, and GAIA propose new benchmarks that cover more diverse and more complex tasks \cite{ruan2023toolemu, shen2023taskbench, mialon2023gaia}. Despite the increase in diversity and complexity in these benchmarks, they lack fully executable solutions and thus fail to support the evaluation of end results, which could be crucial in cases where multiple plans are equally plausible.  

In addition to the differences in task space and evaluation, prior works also formulate task planning differently. While ReACT and ToolLlama formulate it as local planning (i.e. step-by-step prediction) \cite{yao2023react, qin2023toolllm}, VisProg and HuggingGPT treat it as a global planning (i.e. multi-step prediction) problem \cite{shen2023hugginggpt, gupta2022visual}. Tool use is also formulated differently often either as (pseudo-)code generation \cite{gupta2022visual, suris2023vipergpt} or natural language generation following some specific format such as json \cite{shen2023hugginggpt}. Moreover, some works incorporate tool execution feedback into planning \cite{yao2023react, qin2023toolllm} while the others consider execution a different phase \cite{shen2023hugginggpt, gupta2022visual, suris2023vipergpt}. 

All of these differences make it hard to compare existing task planning approaches apple by apple. We wonder: what are the best practices in task planning and tool use with large language models? 

To answer this question, we introduce a novel benchmark M\&Ms (Figure \ref{fig:dataset-examples}) with multi-step multi-modal queries and conduct a systematic study of large language models’ task planning and tool use performance on this benchmark. 
Concretely, we make the following three contributions:
\begin{enumerate}
    \item We contribute a new benchmark with 4k+ multi-step multi-modal queries and 882 human-verified plans in two formats - json and Python code - for solving these queries. These open-ended queries require 1-3 tools among 33 ones across three domains – multimodal ML models, public APIs, and data processing modules to solve;
    % 2) it supports evaluation of planners on ambiguous requests by adding alternative plans to the label set;
    \item We establish a unified evaluation framework to systematically study large language models' task planning and tool use performance in different settings: single-step vs. multi-step prediction, natural language vs. code generation, and without vs. with external feedback;
    \item With this novel dataset and comprehensive framework, we benchmark \modelnum state-of-the-art instruction-tuned large language models with varying sizes to plan over complex multi-modal tasks and solve them.
\end{enumerate}
Through extensive experiments, we learned the following X takeaways: first, global planning leads to better performance than local planning with fewer tokens; second, both verification and execution feedback can improve large language models' performance by 1-3\%; third, something about code vs. json-format natural language generation.  





==> old_sections/02_related_v1.tex <==
\section{Related Work}
\input{tables/benchmark_comparison}

Tool-use and planning has been recognized as an important direction for computer vision research, with CVPR 2023's best paper awarded to a tool-use paper~\cite{gupta2022visual}. Since then, a number of 
 
% Over the last year, several planning agent variants have been proposed.
% For instance, VisProg and ViperGPT evaluate plan \textit{executions} on vision tasks using plans in the form of python-like modular \textit{code}~\cite{gupta2022visual,suris2023vipergpt}.
% HuggingGPT evaluates only the \textit{planning} accuracy (did the agent choose the right tools) without executing the proposed plans~\cite{shen2023hugginggpt}.
% Meanwhile, ToolFormer~\cite{schick2024toolformer} and ToolLLaMA~\cite{qin2023toolllm} both use \textit{natural language} instead of \textit{code} to interface with tools; while ToolFormer generates a \textit{multi-step} plan all at once and evaluates the program's \textit{execution}, ToolLLaMA  generates the plan \textit{step-by-step}, with \textit{self-feedback} to correct mistakes, and only evaluates the \textit{plans}.
% Unfortunately, no single benchmark evaluates planning agents along this combinatorial design space: evaluating both \textit{plans} and\textit{execution}, both \textit{multi-step} and \textit{step-by-step} planning, interacting with tools using both \textit{natural language} and \textit{code}, with and without different types of \textit{feedback}.

% Making evaluation more dire, all prior work focus on different types of tasks across different benchmarks, each with different tool sets.
% Without a standardized evaluation of these design decisions, its difficult to ascertain the trade-offs between all the design choices.
% Most benchmarks, such as HotpotQA, WebShop, GQA, RefCOCO, and NLVR~\cite{yang-etal-2018-hotpotqa,yao2022webshop,hudson2019gqa,kazemzadeh-etal-2014-referitgame,suhr-etal-2017-corpus}, don't contain ground truth plans, conflating planning errors with execution error.
% By contrast, Recent concurrent benchmarks, such as ToolEmu, TaskBench, and GAIA~\cite{ruan2023toolemu, shen2023taskbench, mialon2023gaia}, contain with ground truth plans but fail to support evaluating the execution of the plans, which could be crucial in cases where multiple plans are equally plausible.
% There is a need for a benchmark that enables studying all these designs under standardized conditions.


\noindent\textbf{Type of tool planning: step-by-step vs. multi-step.}
% Tool-usage~\cite{qin2023tool} is a critical building block for large language model (LLM) agents~\cite{wang2023survey,xi2023rise}.
% It enables LLM agents to obtain real-time data and process multimodal information, thereby largely enhancing the capability of LLMs. 
When dealing with complicated user queries that may contain multimodal data, the LLM agents would have to invoke multiple tools to achieve the goal, which requires LLM agents to devise a tool plan correctly.
Prior works have explored different tool planning strategies, which can be roughly categorized into \emph{step-by-step planning}~\cite{yao2023react,qin2023toolllm,gao2023assistgpt} and \emph{multi-step planning}~\cite{gupta2022visual,suris2023vipergpt,shen2023hugginggpt}.
In particular, the step-by-step planning strategy selects one individual tool at each LLM inference, while multi-step planning devises the overall tool plan in a single shot via either json format or a code snippet.
Unfortunately, these two diverse tool planning strategies have not been systematically compared, and it remains unclear which one is preferable.
In this work, we carefully compare both planning strategies using our \name benchmark with varying open-source and close-source LLMs.
% For instance, VisProg and ViperGPT evaluate plan \textit{executions} on vision tasks using plans in the form of python-like modular \textit{code}~\cite{gupta2022visual,suris2023vipergpt}.
% HuggingGPT evaluates only the \textit{planning} accuracy (did the agent choose the right tools) without executing the proposed plans~\cite{shen2023hugginggpt}.
% Meanwhile, ToolFormer~\cite{schick2024toolformer} and ToolLLaMA~\cite{qin2023toolllm} both use \textit{natural language} instead of \textit{code} to interface with tools; while ToolFormer generates a \textit{multi-step} plan all at once and evaluates the program's \textit{execution}, ToolLLaMA  generates the plan \textit{step-by-step}, with \textit{self-feedback} to correct mistakes, and only evaluates the \textit{plans}.
% To assess different tool planning strategies, researchers have introduced several benchmarks~\cite{ruan2023toolemu, shen2023taskbench,huang2023metatool,qin2023toolllm,zhuang2024toolqa}; we demonstrate the comparison between our \name benchmark and previous ones in the Table~\ref{tab:benchmark_comparison}.
% In particular, the prior benchmark most similar to ours is TaskBench~\cite{shen2023taskbench}, while \name\ differs from it by 1) we explicitly consider alternative plans since different yet equivalent tool plans can address some user queries, ignoring alternative plans can underestimate model performance and 2) our queries are based on real data (e.g., real image) rather than placeholder, grounding the task and making it executable.
% In addition, for each LLM, we carefully benchmark different tool planning strategies and offer a rigorous study of not only LLMs but also the planning strategies used.


\noindent\textbf{The effects of feedback on tool planning.}
LLM agents make mistakes; for example, in the context of tool planning, the LLM agent may invoke a text classification model right after an image generation model with the generated image as input.
Such mistakes can be detected by external verifiers and in turn used to guide LLM agents in the form of feedback.
People have explored various types of feedback for LLM in general~\cite{wang2023survey}.
In particular, environmental feedback, such as observation of a made action~\cite{yao2023react}, code execution results~\cite{wu2023autogen}, and so on~\cite{wang2023voyager, zhu2023ghost, rana2023sayplan,sun2024adaplanner},  can be automatically obtained from the environment that the agent is interacting with and used to inform the agent the current state of the environment; human feedback can effectively make the agent align with the human values and
preferences~\cite{wu2023autogen,huang2022inner} or inform the agent whether the current task is successfully addressed~\cite{zhang2023ecoassistant}; and model feedback is a proxy of human feedback yet obtained from either the LLM itself~\cite{shinn2023reflexion, madaan2024self, miao2023selfcheck} or another LLM~\cite{chen2023interact,wang2023mint}.
However, the effect of feedback on different tool planning strategies has not been systematically studied and remains unclear.
In this work, we focus on two types of generic feedback for tool planning: plan verification feedback and tool execution feedback. The former is provided by our plan verification system and aims to guide the LLM agent to correct its plan if the current plan is invalid, and the latter is to provide the LLM agents with the execution results of the current plan.
We aim to characterize the effect of the feedback on the tool planning of LLM agents by standardized evaluations.



==> old_sections/03_method_v1.tex <==
\section{\name: the benchmark}
To facilitate the study of LLM-powered tool-enabled planning agents for \textit{m}ulti-step \textit{m}ulti-modal tasks, we create the \name benchmark. Besides containing user queries annotated with ground truth plans, to ensure the utility of such a benchmark for studying planning agents that rely on execution feedback, it is paramount that the ground truth plans use realistic and executable tools such that the plan can be executed on user inputs.

Before describing the dataset generation process, we first formalize the tool-planning problem.  Given a tool set $\mathcal{T}$, and the user query $\mathcal{Q}$, the LLM agent is required to produce a plan $\mathcal{P}$ that consists of a sequence of tool invocations $\mathcal{P}=[t_1(\{a^k_1=v^k_1\}_k), t_2(\{a^k_2=v^k_2\}_k), \cdots, t_m(\{a^k_m=v^k_m\}_k)]$, where $t_j$ represents the $j^{th}$ tool in the plan, and $a^{k}_{j}$, and $v^{k}_{j}$ represent tool $t_j$'s $k^{th}$ argument name and value respectively. Note that the output of $t_j$ may be used as argument values for subsequent tools $t_{j+1:m}$. Then, to build a benchmark dataset to evaluate the planning agent, we need to construct the tool set $\mathcal{T}$ as well as a set of $N$ query-plan pairs, i.e., $\{(\mathcal{Q}_{i}, \mathcal{P}_{i})\}_{i\in [N]}$.

We now describe our benchmark creation process in Sec.~\ref{sec:data_gen} and present dataset statistics in Sec.~\ref{sec:data_stats}.
%We introduce \name, a new benchmark to support systematic evaluations of planning agents and tool-use  over \textit{m}ulti-step \textit{m}ulti-modal tasks. 
%\ranjay{Add a sentence here high level details about what such a benchmark should contain. What are the desiderata that you need for a good benchmark? Basically set up expectation so that by the end of the section, the the reader feels like you achieved your desiderate.}

% \subsection{Problem Setup}

% Here, we describe the task \name is built for.
% Specifically, given a set of tools (e.g., machine learning models such as text classifier and image generation model), we aim to fulfill the user's \emph{query} by leveraging LLMs and the tools we have.
% As the user may raise complex queries, the LLMs have to invoke multiple tools to 

\subsection{Dataset generation}~\label{sec:data_gen}
\input{figures/dataset_gen}

% To create this dataset with query-plan pairs, we generate the queries with GPT-4 and construct the plans in a rule-based manner. To guide query generation, we provide a sequence of tools and concrete input examples to GPT-4 and prompt it to output realistic user queries. We use the same input examples and tools to generate groundtruth plans in JSON with a rule-based program. Additionally, we map the JSON-format plans into Python code to support code generation evaluation. Then, we ask three human annotators to verify whether each plan can solve the corresponding user query and obtain a human-verified subset. Finally, we perform data balancing on the human-verified subset to obtain 882 examples for evaluation. 

The data generation process of \name consists of five major steps:
1) We construct a valid tool graph with all the tools and sample a subgraph from it as a sequence of tools;
2) To ground the tool plan, we collect real examples (e.g., images) from existing benchmarks as the input to the tool pan;
3) Then we prompt GPT-4 with the tool graph and concrete input examples to generate realistic user queries with few-shot demonstrations; 
4) We use the same input examples and tools to generate ground truth plans in JSON with a rule-based program. Additionally, we map the JSON-format plans into Python code to support code generation evaluation;
5) Finally, we ask three human annotators to verify whether each plan can solve the corresponding user query and obtain a human-verified subset, followed by a data balancing process to balance the tool plan distribution in the final human-verified subset. 

We describe each of the five main steps of our dataset generation pipeline in additional detail below.
\paragraph{Tool graph sampling} 
We first create a directed graph with all 33 tools as the nodes and valid connections between them as the edges. Each edge represents a valid connection from the source tool node to the target tool node. A connection is valid only if the output of the source tool is a valid input to the target tool. For example, there is an edge between \tool{image classification} and \tool{wikipedia simple search}, because the output of \tool{image classification} - a text label - is a valid input to \tool{wikipedia simple search}.   We then sample subgraphs from the full tool graph to obtain tool sequences with valid dependencies between tools. 

\paragraph{Input example sampling} 
To ground query generation, we also want to provide GPT4 with realistic input examples. We collect real-world examples from the validation sets of 11 existing datasets, including ImageNet~\cite{deng2009imagenet}, SQUAD~\cite{rajpurkar-etal-2016-squad}, Visual Genome~\cite{krishna2017visual}, MagicBrush~\cite{zhang2024magicbrush}, librispeech~\cite{7178964}, and so on to use as the inputs to the tool sequences. For example, if the first tool in a tool sequence is \tool{image classification}, we randomly sample an image (e.g. ``16611.jpg'') from ImageNet as the input and ask GPT-4 to include this input in the generated query (Figure \ref{fig:dataset-gen}). 

\paragraph{Query generation} With a set of tool sequences and input examples to the first tools, we prompt GPT-4 to generate realistic user queries. Concretely, we randomly sample five different input examples for each tool sequence and ask GPT-4 to generate two queries for each tool sequence with the same input (See Appendix for the full prompt). 

\paragraph{Plan generation} For plan generation, we write a rule-based program to generate a plan (i.e. a sequence of tool nodes) for each query.  Each node in the plan contains an id, tool name, and an argument dictionary with this tool's argument names as the keys and argument values as values. We populate each node's id and name based on the sampled tool sequence and fill in the argument names for each tool using a pre-defined metadata document. We also fill in the argument values of the first tool using the input examples and those of subsequent tools using a special notation \node{id}{key}, where id refers to the id of the previous node and key refers to the output key. (To further refine the plans to be even more faithful to queries, we rewrite the argument values of \tool{text generation} and \tool{image generation} (e.g. from ``a shark'' to ``a child-friendly book cover image of a shark'') based on the content in the queries by prompting GPT-4 with the queries and original plans.) 

\paragraph{Human verification} Finally, we perform extensive human verification on all 4427 generated query-plan pairs. We ask three expert annotators (who are undergraduate and PhD students in CS) to rate each query-plan pair with 0 or 1, where 1 indicates that the plan can resolve the query perfectly. We obtain a subset of 1500+ examples on which all three annotators rate 1 and perform further filtering of examples with tools (e.g. \tool{image generation} and \tool{text generation}) that appear a lot more frequently than others. 

It is worth noting that our dataset generation pipeline is largely inspired by TaskBench's method \cite{shen2023taskbench} and similar in the graph sampling and query generation steps. However, we want to highlight three major differences: first, we leverage real-world examples as inputs to the tool sequences (in contrast to TaskBench's ``example.jpg'', ``example.wav'' etc.), which not only grounds the generated queries but also enables execution of the tool sequences and thus experiments with execution feedback and evaluation of outputs; second, we use a rule-based program instead of GPT-4 to obtain the groundtruth plans based on the sampled tool sequences, which eliminates the possibility of hallucinated and incorrect information in the plans; lastly, we conduct human verification on all but not just samples of generated query-plan pairs and distill a human-verified high-quality subset, which we believe enables more rigorous evaluation of tool use methods. 

% \paragraph{Data balancing}

\subsection{Dataset quantity and quality}~\label{sec:data_stats}
\input{tables/dataset_stats}
Overall, \name contains a large quantity of query-plan pairs with diverse multi-modal queries as well as human-verified and executable plans (Table \ref{tab:dataset-stats}). 
Concretely, it consists of a total of 4427 raw examples, where 1565 have been verified to be correct by three annotators. After additional filtering for balanced tool distributions, we are left with 882 examples where 70 are single-tool queries, 159 are two-tool queries, and 653 are three-tool queries. In terms of tools, there are 33 unique tools in total across three different categories, of which 13 are multi-modal machine learning models on HuggingFace, 11 are image processing modules from VisProg~\cite{gupta2022visual}, and 9 are free public APIs from RapidAPI\footnote{https://rapidapi.com/hub}. With these tools, we can generate hundreds of valid tool graphs. Our final dataset includes 317 representative tool graphs, where each graph has multiple queries. We showcase a few representative examples in the dataset in Figure \ref{fig:dataset-examples} (See more examples in the Appendix). 


\section{Planning Agent}
% \input{figures/plan_system}
\input{figures/feedback_types}
Given the user query, the agent must interact with an envi
To systematically evaluate large language model agents' task planning and tool use abilities on our benchmark in different setups, we design a modular planning system with four components -- planner, parser, verifier, and executor -- and implement it with AutoGen's framework~\cite{wu2023autogen}. The planner is the key component and can be instantiated with any large language model. Different from a naive large language model agent, our planner agent can also access a parser, verifier, and executor and incorporate feedback from these modules during planning. The parser parses raw outputs from a large language model into either json or code. The verifier checks if a set of pre-defined rules are satisfied and returns a message accordingly (Figure \ref{fig:feedback-types}). We define the following rules for the verifier: if the predicted tool exists in our provided tool list, if it forms a valid connection with the previous tool, and if the predicted argument names match the ones specified in the metadata document. As for the execution module, it either calls the functions corresponding to the predicted tools or executes the predicted code directly in the case of code generation. In contrast to the verifier's output message, which is specific to the error source, the executor directly returns the error message when the prediction fails to execute. 







